Development of a 3D Digital Twin of the Swalmen Tunnel in the Rijkswaterstaat Project

In an ongoing project, a cooperation between the TU/e and the Dutch Department of Waterways and Public Works (Rijkswaterstaat in Dutch, abbreviated to RWS) is established. The project focuses on investigating applicability of synthesis-based engineering in the design of supervisory controllers for bridges, waterways and tunnels. Supervisory controllers ensure correct cooperation between components in a system. The design process of these controllers partly relies on simulation with models of the plant (the physical system). A possible addition to this design process is digital twin technology. A digital twin is a virtual copy of a system that is generally much more realistic than the 2D simulation models that are currently used for supervisory controller validation. In this report, the development of a digital twin of the Swalmen tunnel that is suitable for supervisory control validation is described. The Swalmen tunnel is a highway tunnel in Limburg, the Netherlands. This case study is relevant, because the Swalmen tunnel will be renovated in 2023 and 2028. These renovation projects include updating controlled subsystems in the tunnel, such as boom barriers and traffic lights, and updating the supervisory controller of the tunnel. The digital twin might be useful to aid the supervisory controller design process in these renovation projects.

==> arXiv upload/tikzlibraryfmbepics.code.tex <==

\RequirePackage{relsize}

\usetikzlibrary{shapes.arrows}
\usetikzlibrary{shapes.misc}

\pgfdeclareshape{document}{
    \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
    \inheritanchorborder[from=rectangle]
    \inheritanchor[from=rectangle]{center}
    \inheritanchor[from=rectangle]{mid}
    \inheritanchor[from=rectangle]{base}
    \inheritanchor[from=rectangle]{north}
    \inheritanchor[from=rectangle]{south}
    \inheritanchor[from=rectangle]{west}
    \inheritanchor[from=rectangle]{east}
    \inheritanchor[from=rectangle]{mid west}
    \inheritanchor[from=rectangle]{base west}
    \inheritanchor[from=rectangle]{north west}
    \inheritanchor[from=rectangle]{south west}
    \inheritanchor[from=rectangle]{mid east}
    \inheritanchor[from=rectangle]{base east}
    \inheritanchor[from=rectangle]{north east} % Is this correct??
    \inheritanchor[from=rectangle]{south east}
    \backgroundpath{% this is new
        % store lower right in xa/ya and upper right in xb/yb
        \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
        \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
        % compute corner of ``flipped page''
        \pgf@xc=\pgf@xb \advance\pgf@xc by-5pt % this should be a parameter
        \pgf@yc=\pgf@yb \advance\pgf@yc by-5pt
        % construct main path
        \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
        \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
        \pgfpathclose
        % add little corner
        \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
    }
}

\definecolor{evalcolor}{rgb}{0.000,0.400,0.800}

% In beamer default to background color, otherwise use white
\providecolor{bg}{named}{white}

\tikzset{
fmbe/.style= {
  , x = 6.5em
  , y = 6.5em
  , node distance = 7em
  , on grid
  , shorten >=1pt
  , every artifact/.style = { draw
                            , minimum size=2.5em
                            , font=\larger
                            }
  , document/.style={ every artifact
                    , shape=document % Warning shape and style overload
                    }
  , model/.style={ every artifact
                 , circle
                 , inner sep=0pt
                 %, rounded rectangle
                 }
  , realization/.style={ every artifact
                       , rectangle
                       }
  , infra/.style = { draw
                   , double arrow
                   , double arrow head extend=1ex
                   %, font=\relsize{-1}
                   %, inner sep=.25ex
                   %, after node path = {
                   %    (\tikzlastnode.south east) edge (\tikzlastnode.south west)
                   %    (\tikzlastnode.north east) edge (\tikzlastnode.north west)
                   %  }
                   }
  , actlb/.style = { above
                   , inner sep=0pt
                   , sharp corners
                   , font=\strut
                   }
  , actlb'/.style = { actlb
                    , anchor=mid
                    , fill=bg
                    , font=
                    , inner sep=2pt
                    }
  , act/.style = { ->
                 , rounded corners
                 , every node/.style = actlb
                 }
  %, evalnode/.style = { draw
  %                    , rectangle
  %                    , rounded corners
  %                    , evalcolor
  %                    }
  %, evalconn/.style = { act
  %                    , evalcolor
  %                    , font=\strut
  %                    , inner sep=0pt
  %                    }
  , eval/.style = { %every node/.style= evalnode
                  %, act
                  , ->
                  , rounded corners
                  , every node/.style = actlb
%                  , dashed
                  , draw
                  , evalcolor
                  , font=\strut
                  , inner sep=0pt
                  }
  , hidden/.style = { %semitransparent
                    , opacity=.5
                    , every node/.append style={fill opacity=1,text opacity=.5}
                    }
  }
}



==> tikzlibraryfmbepics.code.tex <==

\RequirePackage{relsize}

\usetikzlibrary{shapes.arrows}
\usetikzlibrary{shapes.misc}

\pgfdeclareshape{document}{
    \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
    \inheritanchorborder[from=rectangle]
    \inheritanchor[from=rectangle]{center}
    \inheritanchor[from=rectangle]{mid}
    \inheritanchor[from=rectangle]{base}
    \inheritanchor[from=rectangle]{north}
    \inheritanchor[from=rectangle]{south}
    \inheritanchor[from=rectangle]{west}
    \inheritanchor[from=rectangle]{east}
    \inheritanchor[from=rectangle]{mid west}
    \inheritanchor[from=rectangle]{base west}
    \inheritanchor[from=rectangle]{north west}
    \inheritanchor[from=rectangle]{south west}
    \inheritanchor[from=rectangle]{mid east}
    \inheritanchor[from=rectangle]{base east}
    \inheritanchor[from=rectangle]{north east} % Is this correct??
    \inheritanchor[from=rectangle]{south east}
    \backgroundpath{% this is new
        % store lower right in xa/ya and upper right in xb/yb
        \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
        \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
        % compute corner of ``flipped page''
        \pgf@xc=\pgf@xb \advance\pgf@xc by-5pt % this should be a parameter
        \pgf@yc=\pgf@yb \advance\pgf@yc by-5pt
        % construct main path
        \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
        \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
        \pgfpathclose
        % add little corner
        \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
    }
}

\definecolor{evalcolor}{rgb}{0.000,0.400,0.800}

% In beamer default to background color, otherwise use white
\providecolor{bg}{named}{white}

\tikzset{
fmbe/.style= {
  , x = 6.5em
  , y = 6.5em
  , node distance = 7em
  , on grid
  , shorten >=1pt
  , every artifact/.style = { draw
                            , minimum size=2.5em
                            , font=\larger
                            }
  , document/.style={ every artifact
                    , shape=document % Warning shape and style overload
                    }
  , model/.style={ every artifact
                 , circle
                 , inner sep=0pt
                 %, rounded rectangle
                 }
  , realization/.style={ every artifact
                       , rectangle
                       }
  , infra/.style = { draw
                   , double arrow
                   , double arrow head extend=1ex
                   %, font=\relsize{-1}
                   %, inner sep=.25ex
                   %, after node path = {
                   %    (\tikzlastnode.south east) edge (\tikzlastnode.south west)
                   %    (\tikzlastnode.north east) edge (\tikzlastnode.north west)
                   %  }
                   }
  , actlb/.style = { above
                   , inner sep=0pt
                   , sharp corners
                   , font=\strut
                   }
  , actlb'/.style = { actlb
                    , anchor=mid
                    , fill=bg
                    , font=
                    , inner sep=2pt
                    }
  , act/.style = { ->
                 , rounded corners
                 , every node/.style = actlb
                 }
  %, evalnode/.style = { draw
  %                    , rectangle
  %                    , rounded corners
  %                    , evalcolor
  %                    }
  %, evalconn/.style = { act
  %                    , evalcolor
  %                    , font=\strut
  %                    , inner sep=0pt
  %                    }
  , eval/.style = { %every node/.style= evalnode
                  %, act
                  , ->
                  , rounded corners
                  , every node/.style = actlb
%                  , dashed
                  , draw
                  , evalcolor
                  , font=\strut
                  , inner sep=0pt
                  }
  , hidden/.style = { %semitransparent
                    , opacity=.5
                    , every node/.append style={fill opacity=1,text opacity=.5}
                    }
  }
}


